The Information Autoencoding Family: A Lagrangian Perspective on Latent Variable Generative Models

A large number of objectives have been proposed to train latent variable generative models. We show that many of them are Lagrangian dual functions of the same primal optimization problem. The primal problem optimizes the mutual information between latent and visible variables, subject to the constraints of accurately modeling the data distribution and performing correct amortized inference. By choosing to maximize or minimize mutual information, and choosing different Lagrange multipliers, we obtain different objectives including InfoGAN, ALI/BiGAN, ALICE, CycleGAN, beta-VAE, adversarial autoencoders, AVB, AS-VAE and InfoVAE. Based on this observation, we provide an exhaustive characterization of the statistical and computational trade-offs made by all the training objectives in this class of Lagrangian duals. Next, we propose a dual optimization method where we optimize model parameters as well as the Lagrange multipliers. This method achieves Pareto optimal solutions in terms of optimizing information and satisfying the constraints.

==> cmd.tex <==
\usepackage[utf8]{inputenc}
\usepackage{float}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{graphicx}
\usepackage{wrapfig}
% \usepackage{subcaption}
\usepackage{placeins}
\usepackage{hyperref}
\usepackage[english]{babel}
\usepackage{url}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{wrapfig}
\usepackage{bm}
\usepackage{psfrag}
\usepackage{tikz}
\usepackage{epstopdf}
\usepackage{xcolor}
\usepackage{adjustbox}

\newcommand{\beq}[1][\vspace{0.3em}]{#1\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\rbx}[2][!]{
	\resizebox{#1}{!}{$#2$}	
}
\newcommand{\eqs}[1]{\begin{align}#1\end{align}}
\newcommand{\mat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bit}{\vspace{0mm}\begin{itemize}}
\newcommand{\eit}{\vspace{0mm}\end{itemize}}
\newcommand{\ben}{\vspace{0mm}\begin{enumerate}}
\newcommand{\een}{\vspace{0mm}\end{enumerate}}
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}

\newcommand{\Av}[0]{{{\bf A}}}
\newcommand{\Bv}[0]{{{\bf B}}}
\newcommand{\Cv}[0]{{{\bf C}}}
\newcommand{\Dv}[0]{{{\bf D}}}
\newcommand{\Ev}[0]{{{\bf E}}}
\newcommand{\Fv}[0]{{{\bf F}}}
\newcommand{\Gv}[0]{{{\bf G}}}
\newcommand{\Hv}[0]{{{\bf H}}}
\newcommand{\Iv}[0]{{{\bf I}}}
\newcommand{\Jv}[0]{{{\bf J}}}
\newcommand{\Kv}[0]{{{\bf K}}}
\newcommand{\Lv}[0]{{{\bf L}}}
\newcommand{\Mv}[0]{{{\bf M}}}
\newcommand{\Nv}[0]{{{\bf N}}}
\newcommand{\Ov}[0]{{{\bf O}}}
\newcommand{\Pv}[0]{{{\bf P}}}
\newcommand{\Qv}[0]{{{\bf Q}}}
\newcommand{\Rv}[0]{{{\bf R}}}
\newcommand{\Sv}[0]{{{\bf S}}}
\newcommand{\Tv}[0]{{{\bf T}}}
\newcommand{\Uv}[0]{{{\bf U}}}
\newcommand{\Vv}[0]{{{\bf V}}}
\newcommand{\Wv}[0]{{{\bf W}}}
\newcommand{\Xv}[0]{{{\bf X}}}
\newcommand{\Yv}[0]{{{\bf Y}}}
\newcommand{\Zv}[0]{{{\bf Z}}}

\newcommand{\av}[0]{{{\bf a}}}
\newcommand{\bv}[0]{{{\bf b}}}
\newcommand{\cv}[0]{{{\bf c}}}
\newcommand{\dv}[0]{{{\bf d}}}
\newcommand{\ev}[0]{{{\bf e}}}
\newcommand{\fv}[0]{{{\bf f}}}
\newcommand{\gv}[0]{{{\bf g}}}
\newcommand{\hv}[0]{{{\bf h}}}
\newcommand{\iv}[0]{{{\bf i}}}
\newcommand{\jv}[0]{{{\bf j}}}
\newcommand{\kv}[0]{{{\bf k}}}
\newcommand{\lv}[0]{{{\bf l}}}
\newcommand{\mv}[0]{{{\bf m}}}
\newcommand{\nv}[0]{{{\bf n}}}
\newcommand{\ov}[0]{{{\bf o}}}
\newcommand{\pv}[0]{{{\bf p}}}
\newcommand{\qv}[0]{{{\bf q}}}
\newcommand{\rv}[0]{{{\bf r}}}
\newcommand{\sv}[0]{{{\bf s}}}
\newcommand{\tv}[0]{{{\bf t}}}
\newcommand{\uv}[0]{{{\bf u}}}
\newcommand{\vv}[0]{{{\bf v}}}
\newcommand{\wv}[0]{{{\bf w}}}
\newcommand{\xv}[0]{{{\bf x}}}
\newcommand{\yv}[0]{{{\bf y}}}
\newcommand{\zv}[0]{{{\bf z}}}
\newcommand{\epsilonv}[0]{{{\bf \epsilon}}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\mb}[1]{\mbox{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}

\providecommand{\abs}[1]{\,\lvert#1\rvert\,}
\providecommand{\norm}[1]{\,\lVert#1\rVert \,}
\newcommand{\Var}{\operatorname{Var}}

\newcommand{\Lim}[1]{\raisebox{0.5ex}{\scalebox{0.8}{$\displaystyle \lim_{#1}\;$}}}

\providecommand{\tightlist}{%
	\setlength{\itemsep}{2pt}\setlength{\parskip}{2pt}}

\providecommand{\js}[1]{{\color{red} [JS: #1]}}
\providecommand{\s}[1]{{\color{blue} [SE: #1]}}
\providecommand{\se}[1]{{\color{blue} [SE: #1]}}
\providecommand{\dl}[1]{{\color{purple} [DL: #1]}}

==> enumeration.tex <==
\section{Enumeration of Tractable Families}
In the previous section, we introduced a very broad family of training objectives encompassing several widely used approaches. While all the objectives in the family are reasonable, the special cases we have identified have a very special property in common: they are (in a certain sense) `easy' to optimize. This is a highly non-trivial property to have. In fact, mutual information and most divergences used in Definition \ref{def:information_autoencoding_family} are generally \emph{not} tractable to compute and/or optimize. Thus, the objectives will be `easy' to optimize only if we carefully choose certain values of the Lagrange multipliers $\lambda_i$, so that certain terms `cancel out'.

In this section, we propose a general framework to formally characterize \emph{all training objectives in the family that satisfy certain tractability requirements}. We formalize tractability by defining the notion of a tractable ``tool box'', corresponding to a set of terms that we assume can be computed/optimized reasonably well, such as the ones used in ELBO \citep{autoencoding_variational_bayes2013,variational_dbn_stochastic_bp2014}, InfoGAN \citep{infogan2016}, InfoVAE \citep{infovae2017}, etc. Note that these objectives are generally not \emph{provably} tractable to optimize, as they involve non-convexities, expectations over high-dimensional spaces, etc. There is, however, significant empirical evidence that they can be optimized reasonably well in practice, and we therefore group them based on the techniques employed. %\s{cite a bunch of stuff here}  

The main technical challenge is dealing with all the possible simplifications and transformations that leave an objective invariant. For example, we need to account for objectives like (\ref{eq:betaelbo2}), which appear to involve components that are difficult to estimate such as $I_q(x; z)$, but can actually be simplified to a more manageable form (\ref{eq:betaelbo}) that can be optimized in a likelihood-based way.%\s{how? likelihood based or free?}.
We therefore define a set of transformations that leave an objective equivalent according to the following definition.
\begin{definition}
\label{def:equivalence}
An objective $\mathcal{L}$ is equivalent to $\mathcal{L}'$ when $\exists C$, so that for all parameters $\theta, \phi$, $\mathcal{L}(\theta, \phi) = \mathcal{L}'(\theta, \phi) + C$. We denote this as $\mathcal{L} \equiv \mathcal{L}'$. %\js{how is $p_{\theta_1}$ eqiv to $p_{\theta_2}$ if parameter size not same?}
\end{definition}
We are then able to analyze all the objectives that contain elements from a given ``tool box", and all objectives derived from them through equivalent transformations. %\rs{Add scaling? Be mindful the current definition of equivalent objectives differ from Boyd's.}
%then define a grammar for the generation of tractable objectives.


%are tractable in a certain sense. satisfying those requirements. 

% \s{this definition seems more confusing that it needs to be?}
% \begin{definition}
% \label{def:information_preference}
% \textbf{Information Preference}: For any two solutions $p_1^*, q_1^*$, and $p_2^*, q_2^*$ that satisfy optimality condition, and $I_{q_1^*}(x; z) \leq I_{q_2^*}(x; z)$, an unbiased optimization objective $\mathcal{L}(p, q)$ is information maximizing if $\mathcal{L}(p_1^*, q_1^*) < \mathcal{L}(p_2^*, q_2^*)$ always holds, information minimizing if $\mathcal{L}(p_1^*, q_1^*) > \mathcal{L}(p_2^*, q_2^*)$, and information neutral otherwise.
% \end{definition}

\subsection{Likelihood-based and likelihood-free Components}
% \js{this is iterating the point in second paragraph of sec 3. should trim, or at least remove references.}
% Given infinite computation and data, any mutual information or divergence can be in principle be optimized. However, different terms may have drastically different computational cost. Past research %\citep{autoencoding_variational_bayes2013,gradient_estimation2015,variational_dbn_stochastic_bp2014,generative_adversarial_nets2014,f_gan2016,wgan2017,ali2016,bigan2016} 
% have identified certain terms as ``easy'' to estimate and optimize over. We define such terms in the following definition.
We formalize the idea of "computation toolbox" by the following definition:

\begin{definition}
\label{def:tractable_families}
For any divergence $D$, we define

\textbf{(1)} Likelihood-based terms as following set
\begin{align*} 
T_1 = \lbrace &\E_p[\log p(x|z)],\E_p[\log p(x, z)],\E_p[\log p(z)],\E_p[\log q(z|x)] \\  
&\E_q[\log p(x|z)],\E_q[\log p(x, z)],\E_q[\log p(z)],\E_q[\log q(z|x)] \rbrace
\end{align*}

\textbf{(2)} Unary likelihood-free terms as the following set
\begin{align*} 
T_2 = \lbrace D(q(x)\Vert p(x)), D(q(z)\Vert p(z)) \rbrace
\end{align*}

\textbf{(3)} Binary likelihood-free terms as the  following set
\begin{align*}
T_3 = \lbrace D(q(x, z)\Vert p(x, z)) \rbrace
\end{align*}

Define an objective $\mathcal{L}$ as likelihood-based computable if there exists equivalent transformations $\mathcal{L}' \equiv \mathcal{L}$ so that $\mathcal{L}'$ only contains terms in $T_1$; unary likelihood-free computable if $\mathcal{L}'$ only contains terms in $T_1 \cup T_2$; binary likelihood-free computable if $\mathcal{L}'$ only contains terms in $T_1 \cup T_2 \cup T_3$.
\end{definition}
%\s{the sentences in this definition are not even complete..you need to say. let likelihood based terms be this set. let unary likelihood free terms be that.. }
%This definition attempts to capture the difficulty of computing and optimizing each of these terms. 

Consider the set $T_1$ of likelihood-based terms. Because we can directly compute likelihoods for $\log p(x|z)$, $\log p(x, z)$, $\log p(z)$ and $\log q(z|x)$, optimizing over an expectation over these terms can be achieved by back-propagation using path-wise derivative methods (the reparameterization trick)~\citep{autoencoding_variational_bayes2013,gradient_estimation2015,gumbel_softmax2016,concrete2016}, and by likelihood ratios when reparameterization is not applicable~\citep{mnih2014neural,gradient_estimation2015}. %\js{also cite concrete and REBAR?} %\s{be more precise. what if they are discrete? things that can be computed via monte carlo, autodiff, baselines, likelihood ratios, etc}

Likelihood-free methods have been extensively studied in recent years. Examples include Jensen Shannon divergence%$JS(p\Vert q)$
~\citep{generative_adversarial_nets2014}, f-divergences~\citep{f_gan2016},
Wasserstein distance~% $W(p\Vert q)$
\citep{wgan2017,improved_wgan2017} and Maximum Mean Discrepancy~\citep{mmd_statistics2007,generative_moment_matching_network2014}. Even though such models are still difficult to train, significant improvements have been made in terms of stability and efficiency. 
%\s{this is not really a single variable. its a group of variables, so no different from the one below..}
Here, we distinguish between the (unary) case,  where we consider a single group of variable at a time (either $x$ or $z$), and the more general binary case.
%In the most general form, we assume a toolbox where we can optimize divergences over implicitly defined models (Binary likelihood-free computable) \citep{ali2016, bigan2016}. 
The reason is that the binary case has been empirically shown to be more difficult to train, for example leading to inaccurate inference~\citep{ali2016, bigan2016}.% \js{if you match the binary divergences it does not require inference between z and x right?}
%\vk{I would try to make the section until now less verbose}

%Therefore we have categorized a hierarchy of computable terms, from the most well studied and easiest to compute (likelihood based computable) to the most general but more difficult to compute (binary likelihood free computable). Now we can proceed to define transformations to extend the basic terms into families of models.

\subsection{Elementary Transformations}

%\s{give some intuition for these transformations. especially the last two (no dep on paramters)}
%\js{maybe can trim if space is not enough}
Many elementary probabilistic identities can be used to rewrite an objective into another one which is equivalent according to Definition \ref{def:equivalence}.
%make two objectives exactly equivalent. 
An example is the chain rule identity
\[ p(x, z) = p(x)p(z|x) = p(z)p(x|z) \]
%which relates joint probability with conditional probability.
%, but also encompasses Bayes formula.
In addition, terms that do not contain trainable parameters ($\phi,\theta$) can be freely added to the objective without affecting the optimization. 
%Such terms will be treated as a constant, and also leaves the objective equivalent. 
Examples include $\Eb_{p}[\log p(z)]$ and $\Eb_q[\log q(x)]$. We formalize the above intuition in the following definition.
\begin{definition}
\label{def:elementary_transformation}
Define the following set of transformations as the elementary transformations
\begin{align*}
\E_*[\log p(x, z)] &\equiv \E_*[\log p(x) + \log p(z|x)] \equiv \E_*[\log p(z) + \log p(x|z)] \\
\E_*[\log q(x, z)] &\equiv \E_*[\log q(x) + \log q(z|x)] \equiv \E_*[\log q(z) + \log q(x|z)] \\
\E_q[\log q(x)] &\equiv 0 \,\qquad \E_p[\log p(z)] \equiv 0
\end{align*}
where $\E_*$ indicates that the equivalence holds for both $\E_p$ and $\E_q$.
\end{definition}
Note that this set does not contain all possible transformations, such as importance sampling
\[ \E_q[\log p(x)] \equiv \E_{q(x)}\left[ \log \E_{q(z|x)}\left[ \frac{p(x, z)}{q(z|x)} \right] \right] \]
%and others based on importance sampling, that are not captured by our analysis. 
%However such transformations involves terms that are difficult to compute. Furthermore we shall show in the next section that the grammar we defined so far is log linear, so we can analytically compute a basis for all possible solutions. 
We leave extensions to more general transformations to future work. Nevertheless, we are now in a position to study \emph{all} the objectives that can be constructed using the building blocks from Definition \ref{def:tractable_families}, and any objective derived by applying elementary transformations.
%analyzing their tractability and other properties up to elementary transformations.
From now on, we restrict the definition of tractable family in Definition~\ref{def:tractable_families} to equivalence by elementary transformation only. 
%all objectives that can be transformed by elementary transformations to only contain terms in corresponding computable categories. 
%\vk{I think this section is also a bit too verbose}
% \textbf{Tractable to compute (explicit):} $p(x|z)$, $q(z|x)$, $p(z)$, $p(x, z)$, 

% \textbf{Tractable to sample (implicit):} $q(x)$, $q(z)$, $p(x)$, $q(x, z)$

% \textbf{Intractable:} $q(x|z)$, $p(z|x)$

% \s{relate this to implicit vs explicit models}




% \subsubsection{Likelihood-Free Optimization}
% For these methods we only have to eliminate all terms that are intractable to sample from, namely for this case, $q(x|z)$ and $p(z|x)$
% \begin{align*}
% &\mathcal{L}_{VAE1} \\ 
% &= E_{p(x, z)}\left[ \log \frac{p(z, x)^{\lambda_2} p(x|z)^\beta p(x)^{\lambda_1-\lambda_2-\beta}}{q(x, z)^{\lambda_2+\beta} q(z|x)^{-\beta} q(x)^{\lambda_1-\lambda_2-\beta}} \right] \numberthis \label{equ:form11} \\
% &= E_{p(x, z)}\left[ \log \frac{p(x|z)^{\lambda_2+\beta} p(x)^{\lambda_1-\lambda_2-\beta}}{q(z|x)^{\lambda_2}q(x)^{\lambda_2 + \beta}q(x)^{\lambda_1-\lambda_2-\beta}} \right] \numberthis \label{equ:form12}
% \end{align*}
% \begin{align*}
% &\mathcal{L}_{VAE2} \\
% &= E_{q(x, z)}\left[ \log \frac{q(z, x)^{\lambda_2} q(z|x)^\beta q(z)^{\lambda_1-\lambda_2-\beta}}{p(x, z)^{\lambda_2}p(z)^{\beta}p(z)^{\lambda_1-\lambda_2-\beta}} \right] \numberthis \label{equ:form21} \\
% &= E_{q(x, z)}\left[ \log \frac{q(z|x)^{\lambda_2+\beta} q(z)^{\lambda_1-\lambda_2-\beta}}{p(x|z)^{\lambda_2}p(z)^{\lambda_2 + \beta}p(z)^{\lambda_1-\lambda_2-\beta}} \right] \numberthis \label{equ:form22}
% \end{align*}
% The first forms (\ref{equ:form11}) (\ref{equ:form21}) corresponds with ALI or Bi-GAN, while the second form (\ref{equ:form12}) (\ref{equ:form22}) removes the use of likelihood free \js{check this} optimization of $KL(p(x, z)||q(x, z))$, which has been observed to lead to inaccurate inference. 

% All of the first forms (\ref{equ:form11}) (\ref{equ:form21}) can be computed likelihood-free for any choice of $\beta, \lambda_1, \lambda_2$. However, there is an asymmetriy between $x$ and $z$ for second form, where $p(x, z)$ is tractable to compute, while $q(x, z)$ is only tractable to sample. Therefore, (\ref{equ:form22}) is tractable for all $\beta, \lambda_1, \lambda_2$, while (\ref{equ:form12}) is only tractable when $\lambda_2+\beta = 0$. Because $\lambda_2 > 0$, we must have $\beta < 0$, that is, form (\ref{equ:form12}) can only be used to maximize information. 


\subsection{Enumeration of KL Information-Autoencoding Family}

%\s{say somewhere that we are restricted to KL}

In the previous sections we have formally defined a grammar for tractable models. In this section, we will use these definitions to find all possible objectives that can be optimized under given tractability assumptions. We shall write the largest family under each tractability constraint in two forms: a Lagrangian dual form, and an equivalent tractable form that only contains terms satisfying assumed computability constraints. 

In this section we focus on the KL Information-Autoencoding family defined in Definition~\ref{def:information_autoencoding_family} where all divergences in the constraints are either $\KL$ or $D_{\neg \mathrm{KL}}$.\footnote{To avoid cluttering the notation, if a $\KL$ term has free variables such as $z$ in $\KL(q(x|z)\Vert p(x|z))$, then we take the expectation for that free variable with respect to $p$ when the first distribution of the KL divergence is $\KL(p \Vert \cdot)$, and with respect to $q$ otherwise, e.g. $\E_{q(z)}[\KL(q(x|z)\Vert p(x|z))]$, $\E_{p(z)}[\KL(p(x|z)\Vert q(x|z)]$.} We discuss KL divergence because it is the most interesting case to study under elementary transformations. KL divergence is a sum of expectations over log probabilities $ \KL(p||q) = \Eb_p[\log p - \log q] $
while the elementary transformations are all linear operations on log probabilities. We will discuss generalization to other divergences in the next section. 
%We shall make the following definition, and show that most existing models are not only special cases of our general formulation, but also \textbf{unique} tractable families under mild assumptions.
%\shengjia{Example of new model equivalent to old model, on both directions of transformation}


%\vk{Until here, this subsection sounds like a review of what is KL, and I don't think I received any new information from it}

%\s{break down this theorem, and add discussion. explain in words, and discuss significance}
%\s{mention f-gans?}
%\s{beta,lambas are confusing}
%\js{maybe should mention what $\beta$ is used in the thms.}

For likelihood based computable families, we show that variational mutual information maximization \citep{variational_infomax2003} and $\beta$-ELBO \citep{beta_vae2016} are the only possible families (up to equivalences). Based on the set of transformations we considered, there do not exist other objectives satisfying the stated computational constraints. This is formally given by the following theorem.
%\s{i wonder if the statement is accurate. likelihood based computable is defined in terms of \textbf{any} transformation. but the proof is really only over elementary ones. double check very carefully the wording!}\shengjia{fixed by a statement at end of sec 3.2}
\begin{theorem}
\label{thm:elementary_equivalence1}
Define the following objectives

\textbf{1)} Variational mutual information maximization %\js{do you need the expectation at third line?}
\begin{align*}
\mathcal{L}_{\mathrm{VMI}} = -I_p(x; z) + \KL(p(z|x)\Vert q(z|x)) = \E_p[\log q(z|x)]
\end{align*}
\textbf{2)} $\beta$-ELBO, where $\beta$ is any real number
\begin{align*}
\mathcal{L}_{\beta-\mathrm{VAE}} &= (\beta - 1) I_q(x, z) + \KL(q(x|z)\Vert p(x|z)) + \beta \KL(q(z)\Vert p(z)) \\
&= - \E_{q}[\log p(x|z)] + \beta \E_q[\log q(z|x)] - \beta \E_q[\log p(z)] %\KL(q(z|x)\Vert p(z))
\end{align*}
Then any likelihood based computable objective of the KL Info-Autoencoding family is equivalent by elementary transformation to a linear combination of $\mathcal{L}_{\beta-\mathrm{ELBO}}$ and $\mathcal{L}_{\mathrm{VMI}}$. %\js{likelihood based appears at def 5 sec 3; KLVAE family appears at def 5 sec 2. I can understand, but it requires looking back and forth. I would suggest modifying def 7 such that we mention KLAE in def 5, so readers would not already have forgot about KLVAE family.}
\end{theorem}

%\vk{Some short proof sketch or general idea of why it's true would be useful here (you could shorten earlier sections to make space)}
We formally prove this theorem in the appendix and give a brief sketch here. This theorem is proved by demonstrating that a set of terms such as $\E_q[\log p(x)]$ can be selected, so that each objective of the KL Information-Autoencoding family is a linear combination of these basic terms. Treating the set of basic terms as basis for a vector space (over functions), each training objective can be represented as a vector in this space. Each family of objectives can be represented as a subset and in some cases as a linear subspace. The key technical difficulty is to show that the following family of objectives correspond to the same linear subspace:

1. Linear combinations of $\mathcal{L}_{\beta-\mathrm{ELBO}}$ and $\mathcal{L}_{\mathrm{VMI}}$, and their elementary transformations.

2. Likelihood-based objectives (as in Definition~\ref{def:tractable_families}), and their elementary transformations.
%\s{does not sound intuitive to me}

For unary likelihood free computable objectives, we show that a slight generalization of InfoGAN and InfoVAE are the only possible families. This is formally given by the following theorem.
\begin{theorem}
\label{thm:elementary_equivalence2}
Define the following objectives

\textbf{3)} KL InfoGAN, where $\lambda_1, \lambda_2$ are any real number
\begin{align*}
\mathcal{L}_{\mathrm{InfoGAN}} &= - I_p(x; z) + \KL(p(z|x)\Vert q(z|x)) + \lambda_1 \KL(p(x)\Vert q(x)) + \lambda_2 \KL(q(x)\Vert p(x)) \\
&= - \E_p[\log q(z|x)] + \lambda_1 \KL(p(x)\Vert q(x)) + \lambda_2 \KL(q(x)\Vert p(x))
\end{align*}
\textbf{4)} KL InfoVAE, where $\alpha, \lambda_1, \lambda_2$ are any real number
\begin{align*}
\mathcal{L}_{\mathrm{InfoVAE}} &= \alpha I_q(x; z) + \KL(q(x|z)\Vert p(x|z)) + \lambda_1 \KL(q(z)\Vert p(z)) + \lambda_2 \KL(p(z)\Vert q(z)) \\
&= - \E_{q}[\log p(x|z)] +  (\alpha + 1) \E_q[\log q(z|x)] - (\alpha + 1) \E_q[\log p(z)] + \\
& \qquad (\lambda_1 - \alpha - 1) \KL(q(z)\Vert p(z)) + \lambda_2 \KL(p(z)\Vert q(z))
\end{align*}
Then any unary likelihood free computable objective of the KL Info-Autoencoding family is equivalent by elementary transformation to a linear combination of $\mathcal{L}_{\mathrm{InfoGAN}}$ and $\mathcal{L}_{\mathrm{InfoVAE}}$.
\end{theorem}
Note that there is a slight asymmetry between InfoGAN and InfoVAE because $\log q(x)$ is assumed to be intractable, while $\log p(z)$ is assumed tractable. The consequence is that for InfoGAN, the coefficient for the mutual information term $I_p(x; z)$ must be tied together with the coefficient for $\KL(q(x|z)\Vert p(x|z))$ to meet the computational constraint. This means that InfoGAN can only maximize mutual information. On the other hand, InfoVAE can either maximize or minimize mutual information.

Finally for the most general case, we show that any binary likelihood free computable member of the KL Information-Autoencoding family can be written as a linear combination of InfoVAE and an information maximizing/minimizing form of BiGAN/ALI/ALICE \citep{bigan2016,ali2016,alice2017}, which we term InfoBiGAN.
\begin{theorem}
\label{thm:elementary_equivalence3}
Define the following objective

\textbf{5)} KL InfoBiGAN, where $\alpha, \lambda_1, \lambda_2$ are any real number 
\begin{align*}
\mathcal{L}_{\mathrm{InfoBiGAN}} &= \alpha I_p(x; z) + \KL(p(z|x)\Vert q(z|x)) + \lambda_1 \KL(p(x)\Vert q(x)) + \lambda_2 \KL(q(x)\Vert p(x)) \\
&= (\alpha + 1) \KL(p(x, z)\Vert q(x, z)) + (\lambda_1 - \alpha - 1) \KL(p(x)\Vert q(x)) + \\
&\qquad \lambda_2 \KL(q(x)\Vert p(x)) - \alpha \E_p[\log q(z|x)]
\end{align*}
Then any binary likelihood free computable objective of the KL Info-Autoencoding family is equivalent by elementary transformation to a linear combination of $\mathcal{L}_{\mathrm{InfoVAE}}$ and $\mathcal{L}_{\mathrm{InfoBiGAN}}$.
\end{theorem}
%\shengjia{TODO: Double check signs}


\subsection{Extensions and Limitations}
A simple extension beyond KL divergence is possible. For any KL Info-Autoencoding family under the given tractability assumptions, we may add terms in the same tractability category and the resulting objective will still satisfy the same tractability assumptions. For example, for a subset of the KL InfoVAE family, we can add the Maximum Mean Discrepancy (MMD) distance to derive the MMD InfoVAE \citep{infovae2017} in Lagrangian form. 
\[ \mathcal{L}_{\mathrm{MMD-VAE}} = \alpha I_q(x; z) + \KL(q(x|z)\Vert p(x|z)) + \lambda D_{\mathrm{MMD}}(p(z) \Vert q(z)) \]
and this will still be unary likelihood free computable. 

There are two limitations to our analysis. First we do not prove uniqueness results for families with arbitrary divergences. Second we use restricted computability toolboxes and elementary transformations. More general results could be derived by considering a broader family of divergences, computable terms, and transformations. For example, enumeration for models including Renyi divergence variational inference \citep{renyi_vi2016} and Stein variational gradient \citep{stein_variational2016} are interesting directions for future work.

% if the same term, e.g. $\lambda \KL(p(x)||q(x))$ appear in both forms, we can replace it with another divergence, e.g. $\lambda \JS(p(x)||q(x))$ without breaking the equivalence relationship. \js{why? and using what equivalence? should not be definition 8 right? this seems a bit confusing to me.}



%\vk{I think it would be useful to discuss at some point which models are not in your general family, and hence are not covered by these theorems (just to understand the limits of your work)}

%\vk{I was a little bit confused about why you focus on KL divergences, when it seems like GAN-based methods that use the JS div are part of the examples that you gave earlier. It could be just me.}

